Secrecy: Secure collaborative analytics on secret-shared data

We present a relational MPC framework for secure collaborative analytics on private data with no information leakage. Our work targets challenging use cases where data owners may not have private resources to participate in the computation, thus, they need to securely outsource the data analysis to untrusted third parties. We define a set of oblivious operators, explain the secure primitives they rely on, and analyze their costs in terms of operations and inter-party communication. We show how these operators can be composed to form end-to-end oblivious queries, and we introduce logical and physical optimizations that dramatically reduce the space and communication requirements during query execution, in some cases from quadratic to linear or from linear to logarithmic with respect to the cardinality of the input. We implement our framework on top of replicated secret sharing in a system called Secrecy and evaluate it using real queries from several MPC application areas. Our experiments demonstrate that the proposed optimizations can result in over 1000x lower execution times compared to baseline approaches, enabling Secrecy to outperform state-of-the-art frameworks and compute MPC queries on millions of input rows with a single thread per party.

==> algebra.tex <==
\section{Secure relational algebra}\label{sec:algebra}

==> comparison-table.tex <==
\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{cccccccc}
  \multicolumn{1}{c}{\rot{\textbf{Framework}}} &
  \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}MPC Protocol\end{tabular}}}} &
  %\multicolumn{1}{c}{\rot{\textbf{\#Parties}}} &
%  \multicolumn{1}{c|}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Special \\ Hardware\end{tabular}}}} &
  \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Information \\ Leakage\end{tabular}}}} &
  \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Trusted \\ Party\end{tabular}}}} &
 % \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}MPC Plan \\ Optimization\end{tabular}}}} &
  \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Query \\ Execution\end{tabular}}}} &
  \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Optimization \\ Objective\end{tabular}}}} &
  \multicolumn{1}{c}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Optimization Conditions\end{tabular}}}}
%  \multicolumn{1}{c|}{\rot{\textbf{\begin{tabular}[c]{@{}c@{}}Threat \\ Model\end{tabular}}}}
   \\ \hline
  
  %\multicolumn{1}{|l|}{} &
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Conclave~\cite{Volgushev2019Conclave}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Secret Sharing /\\Garbled Circuits \end{tabular}} &% (w.\\ Sharemind)\end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3 (data owners)\end{tabular} } &
%  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Controlled \\ (Hybrid operators)\end{tabular}} &
  \multicolumn{1}{c|}{Yes} &
 % \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{Hybrid} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Minimize the use of\\ secure computation\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}1. Data owners participate in computation\\ 2. Data owners provide privacy annotations\\ 3. There exists a (fourth) trusted party\end{tabular}}
%  \multicolumn{1}{c|}{SH} 
  \\ \hline
  
 %\multicolumn{1}{|c|}{\multirow{5}{*}{\roty{\textbf{Collaborative Analytics}}}} &
 \multicolumn{1}{|l|}{SMCQL~\cite{Bater2017SMCQL}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Garbled Circuits /\\ORAM \end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2 (data owners)\end{tabular} } &
  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{No} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}$No^{\star}$\end{tabular}} &
 % \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{Hybrid} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Minimize the use of\\ secure computation\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}1. Data owners participate in computation \\ 2. Data owners provide privacy annotations\end{tabular}}
%  \multicolumn{1}{c|}{SH} 
  \\ \hline


  
%  \multicolumn{1}{|l|}{} &
  \multicolumn{1}{|l|}{Shrinkwrap~\cite{bater2018shrinkwrap}} &
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Garbled Circuits /\\ORAM \end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2 (data owners)\end{tabular} } &
%  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Controlled \\ (Diff. Privacy)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}No\end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Yes\\ (Diff. Privacy \\ budget allocation)\end{tabular}} &
  \multicolumn{1}{c|}{Hybrid} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Calibrate padding of\\intermediate results\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\hspace{0.9mm}1. Data owners participate in computation$^1$\\ \hspace{0.9mm}2. Data owners provide privacy annotations$^1$\\ \hspace{0.9mm}and intermediate result sensitivities\end{tabular}}
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Data owners provide sensitivities\\ for intermediate query results$^1$\end{tabular}}
%  \multicolumn{1}{c|}{SH} 
  \\ \hline
  
%  \multicolumn{1}{|l|}{} &
  \multicolumn{1}{|l|}{SAQE~\cite{bater2020saqe}} &
  \multicolumn{1}{c|}{Garbled Circuits} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2 (data owners)\end{tabular} } &
  %\multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Controlled \\ (Diff. Privacy)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}No\end{tabular}} &
 % \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{Hybrid} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Choose sampling rate\\for approximate answers\end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Data owners provide sensitivities\\ for intermediate query results$^1$\end{tabular}}
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\hspace{0.9mm}1. Data owners participate in computation$^1$\\ \hspace{0.9mm}2. Data owners provide privacy annotations$^1$\\ \hspace{0.9mm}and privacy budget \end{tabular}}
%  \multicolumn{1}{c|}{SH} 
  \\ \hline
  
%  \multicolumn{1}{|l|}{} &
  \multicolumn{1}{|l|}{Senate~\cite{Poddar2021Senate} $^{2}$} &
  \multicolumn{1}{c|}{Garbled Circuits} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{k}  (data owners)\end{tabular}} &
%  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{No} &
 \multicolumn{1}{c|}{No} &
  %\multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{Hybrid} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Reduce joint computation\\ to subsets of parties\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\hspace{0.2mm}1. Data owners participate in computation\\ \hspace{0.2mm}2. Input or intermediate relations are owned\\  \hspace{0.2mm}by subsets of the computing parties\end{tabular}}
%  \multicolumn{1}{c|}{M} 
  \\ \hline

%\multicolumn{1}{|l|}{\multirow{3}{*}{\roty{\textbf{Outsourced DBs}}}} &
  \multicolumn{1}{|l|}{SDB~\cite{wong2014secure, he2015sdb} $^{3}$} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Secret Sharing\end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} 1 data owner and \\ 1 untrusted server\end{tabular}} &
%  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Yes \\ (operator dependent)\end{tabular}} &
  \multicolumn{1}{c|}{No} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Yes (Modular \\ exponentials)\end{tabular}} &
  \multicolumn{1}{c|}{Hybrid} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Reduce data encryption\\ and decryption costs\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\hspace{-0.2mm}1. Data owner participates in computation\\ \hspace{-0.2mm}2. Data owner provides privacy annotations\end{tabular}}
%  \multicolumn{1}{c|}{} 
  \\  \hline
  
%  \multicolumn{1}{|l|}{} &
%  \multicolumn{1}{|l|}{StealthDB~\cite{stealthdb}} &
%  \multicolumn{1}{c|}{n/a} &
%  \multicolumn{1}{c|}{1 / No} &
%  \multicolumn{1}{c|}{Yes} &
%  \multicolumn{1}{c|}{No} &
%  \multicolumn{1}{c|}{n/a} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} \\  \cline{2-12} 
  
%  \multicolumn{1}{|l|}{} &
%  \multicolumn{1}{|l|}{Arx~\cote{arx}} &
%  \multicolumn{1}{c|}{n/a} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} \\  \cline{1-12} 
  
%  \multicolumn{1}{l|}{} &
% \multicolumn{1}{|l|}{ObliDB} &
% \multicolumn{1}{c|}{n/a} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{Yes} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} \\  \cline{2-12} 
  
%  \multicolumn{1}{l|}{} &
% \multicolumn{1}{|l|}{Opaque} &
% \multicolumn{1}{c|}{n/a} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{Yes} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} \\ \hline 
  
  \\ \hline
  \multicolumn{1}{|l|}{\textbf{\ours}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Rep. Secret Sharing\end{tabular}} & %\\ (Section~\ref{sec:replicated-sharing})\end{tabular}} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{k} data owners and\\ 3 computing parties\end{tabular}} &
%  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{No} &
  \multicolumn{1}{c|}{No} &
  %\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Yes \\ (Section~\ref{sec:optimizations})\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}End-to-end \\ under MPC\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Reduce MPC costs (\S \ref{sec:optimizations})\end{tabular}} &
  \multicolumn{1}{c|}{None}
%  \multicolumn{1}{c|}{SH} 
  \\ \hline
\end{tabular}
\begin{flushleft}
%\hspace{1mm}\emph{$^{*}$SMCQL-based systems rely on a semi-honest broker.} \\
\hspace{2mm}\emph{$^{1}$ Shrinkwrap and SAQE build on top of SMCQL's information flow analysis and inherit its optimizations along with their conditions.}\\
\hspace{2mm}\emph{$^{2}$ Senate provides security against malicious parties whereas all other systems adopt a semi-honest model.}\\
%\emph{$^2$ Hybrid approaches reveal the intermediate data sizes at the boundary of the plaintext and secure parts of the query plan unless local results are padded.} \\
\hspace{2mm}\emph{$^{3}$ SDB adopts a typical DBaaS model with one data owner and does not support collaborative analytics.} \\
\end{flushleft}
\caption{Summary of MPC-based software solutions for relational analytics. Hybrid query execution is  feasible when data owners participate in the computation. The rest of the optimizations supported by each system are applicable under one or more of the listed conditions.}
\end{table*}\label{tbl:comparison}


==> composition.tex <==

\subsection{Composing oblivious operators}\label{sec:constructing_plans}

We now describe how the oblivious operators in our framework can be put together to construct oblivious query plans.
Since none of the operators reveals anything about its output or access patterns, all operators of Section~\ref{sec:secure_operators} can be arbitrarily combined, as in cleartext evaluation~\cite{10.5555/556863}, to compose an \emph{end-to-end oblivious query} plan without additional special treatment. We regard this as a particular merit of our approach. 

Recall that some oblivious operators introduce a new attribute that stores the result of a logical formula (e.g. the result of the selection predicate). In this case, applying an oblivious operator to the output of another oblivious operator  requires combining the results of these formulas. For example, consider an oblivious equi-join $R\bowtie_{a=c} S$ between two relations $R(a,b)$ and $S(c,d)$. The join generates a relation $T(a,b,c,d,a_\theta)$, where $a_\theta$ denotes the extra attribute that stores the result of the join predicate $\theta$ when applied to the respective pair of tuples. Suppose the join is followed by a selection, e.g. $\sigma_{b=123}(T)$, in the query plan. To perform the selection, we simply apply the selection predicate $\phi$ to each tuple in $T$, compute the logical AND between $\phi$'s and $\theta$'s result bits, and store the result back in $a_\theta$. The logical AND is evaluated under MPC as explained in Section~\ref{}. In this example, the composition requires a logical AND between $\phi$ and $\theta$ but, in general, the logical expression we need to evaluate depends on the query and is inferred (at compile time) from the query syntax. 
This way we compose selections, joins, semi-joins and distinct operators. 

%Compose selection with join and semi-join or distinct: AND bits

%Composition with group-by is based on the same technique. Consider a plan where a selection $\sigma_{a_s=123}(R)$ on relation $R(a_s,a_k)$ is followed by a group-by operator $\gamma_{a_k}$ that applies a \texttt{COUNT(*)} aggregation to each group. The selection produces a relation $T(a_s, a_k, a_\phi)$, where $a_\phi$ stores the result bit of the selection predicate. Applying the group-by operator to $T$ requires identifying only those tuples in $T$ that are selected (i.e. their $a_\phi$ attribute is set) and belong to the same group (i.e. they have the same value for the attribute $a_k$). To do so, the sorting step in group-by needs to take into account $a_\phi$ and sort $R$ first on $a_\phi$ and then on $a_k$. After that, the operator computes a composite bit $b_c~\leftarrow~b~\wedge~t_i[a_\phi]~\wedge~t_{i+1}[a_\phi]$, where $b$ is the equality bit  as in Algorithm~\ref{alg:group}, and uses $b_c$ to aggregate and mask tuples obliviously. The pseudocode is given in Algorithm~\ref{alg:composite_group}. Group-by with aggregation can be applied to a join output similarly.
%
%\john{The composite group-by looks like something standard although it's actually a contribution.}

%\begin{algorithm}[t]
%\small
%%\Input{A stream $S$ of logs and a window $[t_s,t_e]$;}
%%\Output{The graph snapshot $G_{[t_s,t_e]}$;}
%
%%\BlankLine
%
%sort input relation R on $a_\phi$, $a_k$;
%
%%let $a_k$ be the group-by key, $a_w$ the aggregated attribute, and $a_g$ the extra attribute that stores the aggregation result;
%
%\For {each pair of adjacent tuples ($t_i$, $t_{i+1}$), $0\leq i < |R|$,} {
%  
%  \Comment{Are tuples in the same group?}
%  
%  let $b \leftarrow t_i[a_k] \stackrel{?}{=} t_{i+1}[a_k]$;
%  
%   \Comment{Are tuples selected too?}
%    
%  let $b_c\leftarrow b~\wedge~t_i[a_\phi]~\wedge~t_{i+1}[a_\phi]$;
%  
%  \Comment{Aggregation}
%  
%  $t_{i+1}[a_g] \leftarrow b_c\cdot agg\Big(t_i[a_w], t_{i+1}[a_w]\Big) + (1-b_c)\cdot t_{i+1}[a_g]$;
%  
%  \Comment{Masking}
%  \For {each attribute $a$ of $t_i$} {
%  	
%	let $r$ a random value;
%	
%  	$a \leftarrow b_c\cdot r~~+~~(1-b_c)\cdot a$;
%  } 
%  
%  shuffle R; %\Com{Only if there is no subsequent order-by}
%}
%
%%re-distribute $E_h$ based on $(id_{src},id_{dst},id_{corr})$;
%%Pair up half edges in each partition and create the set $E_{comm}$ of edges for communication activities;
%%\textbf{return} $E_w \cup E_{c}$
%\caption{\small Applying group-by to the output of a selection $\sigma_\phi$}\label{alg:composite_group}
%\end{algorithm}

%Compose selection with group-by: create composite bit using the selection bit and the group-by bit
%Compose selection or distinct with sorting: sort by the selected/distinct bit. Nothing special here. 
%Composing join with group-by or distinct
%Composing distinct with group-by on a different attribute (is this possible?)
%Applying sorting to the output of an operator is straight-forward. 

When composing oblivious operators, the additional logical expressions we need to evaluate result in queries whose cost is not equal to the sum of individual operator costs, as in the case of cleartext queries. Although the logical ANDs in the previous examples incur negligible CPU cost, they require communication between parties which increases the total I/O cost of the query. We come back to this issue in Section~\ref{sec:costs}.

%\vasia{Describe how we can combine the operators of the previous section to generate query plans. Define a few composition rules for the different operator categories we define in the previous section. For instance, to compute distinct on the result of a selection, we order by the selected bit first and then compare the neighboring pairs with an additional logical and. This way we avoid a linear scan.}

%The only exception in this general rule is when the query includes an \texttt{ORDER-BY} with a \texttt{LIMIT} clause.
%
%Recall from Section~\ref{sec:secure_operators} that order-by with limit is the only operator that may output a relation with cardinality smaller than the cardinality of its input. In a non-secure plan, limit could be in principle placed early (e.g. right above the leaves) to reduce the size of intermediate data. For example, consider the query below:
%
%\begin{verbatim}
%SELECT pid 
%FROM Diagnosis
%WHERE age=40
%ORDER BY num_visits DESC
%LIMIT 10
%\end{verbatim}
%
%This query asks for the IDs of those ten patients who are 40 years old and have the most visits amongst all other patients. 
%In a non-secure evaluation, the \texttt{ORDER-BY} could be placed 
%and in case the data are not enough, could output more data in a pull-based fashion. In our setting this would reveal information to the computing parties, thus, limit cannot simply output k tuples, unless it the ordering has already taken into account the selected bits of all necessary operators in the plan.
%


==> conclusion.tex <==
\section{Conclusions and Future Work}\label{sec:conclusion}

==> costs.tex <==
\section{Cost analysis}\label{sec:costs}

%\vasia{explain the costs of composition, too, i.e. that it is not additive}

\john{Explain the execution model for the cost analysis: single-thread}

%\begin{table}[h]\scriptsize
%\begin{center}
% \begin{tabular}{||c c c ||} 
% \hline
% Operation & \#operations & \#communication rounds \\ [0.5ex] 
% \hline\hline
%\texttt{Equality} &  $n$ & $\Big\lceil\log\ell\Big\rceil$   \\  % (\texttt{=}) 
%  \hline
% \texttt{Inequality} & 0 & $\Big\lceil\log(\ell+1)\Big\rceil$ \\
% \hline
% \texttt{Addition} & $n\cdot m$ &$\Bigg\lceil\log\Big(3\ell + \frac{\ell(\ell - 1)}{2} + 1\Big)\Bigg\rceil$  \\
%% \hline
%% Range-Join & $n\cdot m$ & $\mathcal{O}(1)$  \\
% \hline
% \texttt{Conversion}& $n\cdot log^2n$ & $\mathcal{O}(n)$  \\ [1ex]
% \hline
%\end{tabular}
%\caption{Costs of primitive MPC operations}
% \label{tab:primitive_costs}
%\end{center}
%\end{table}

In this section we analyze the cost of the MPC operators supported by our framework. We start with primitive operations  in Section~\ref{sec:cost_primitives} and focus on relational operators in Section~\ref{sec:cost_relational}. In Section~\ref{sec:data_overhead}, we discuss the overhead of oblivious operations with respect to the amount of data they exchange. Finally, Section~\ref{sec:optimizations} describes the logical optimizations we introduce to reduce the cost of oblivious queries.

\stitle{Costs.}  Costs are given in terms of CPU and I/O. For relational operators, the CPU cost is defined as the total \emph{number of operations} per party with respect to the input size. The I/O cost refers to inter-party communication and is measured in number of \emph{communication rounds} across parties. A communication round corresponds to a single clockwise data exchange on the ring. In practice, this is a \emph{barrier}, i.e. a synchronization point in the distributed computation, where parties must exchange data in order to proceed. In general, the fewer rounds an operation needs the faster it reaches completion since each party can make more progress in parallel without being blocked on other parties.  All secret-shared data in our framework reside in main memory, therefore, we do not consider disk I/Os.
 
\stitle{Remark.} The analysis we present on communication rounds is valid for other secret-sharing protocols as well. For instance, the only difference between our replicated secret-sharing protocol and other protocols based on Beaver triples~\cite{} \john{Add ref} is the amount of data the parties exchange during computation. In our framework, when a party reaches a barrier, it sends the intermediate data to its successor on the ring and waits for intermediate data from its predecessor (cf. Section~\ref{sec:background}). In the secret-sharing protocol of~\cite{} \john{Add ref}, each party reaches the same barriers but it must instead broadcast its intermediate data to all other parties. 

\ignore{
\subsection{Primitive operations}\label{sec:cost_primitives}

\stitle{Equality/Inequality.} 
%We first analyze the costs of primitive operations, i.e. equality, inequality, addition, conversion, and compare-and-swap. 
%Let $s1$ and $s2$ be two shares of size $\ell$ in number of bits.
The number of rounds for secure equality (=,~<>) and inequality ($<, >, \geq, \leq$) is $\Big\lceil\log\ell\Big\rceil$ and $\Big\lceil\log(\ell+1)\Big\rceil$ respectively, where $\ell$ is the length of the operands in number of bits. For example, to check equality (resp. inequality) between two 64-bit integers using secret sharing, we need $\lceil\log64\rceil=6$ (resp.  $\lceil\log65\rceil=7$) rounds. In most secret-sharing frameworks~\cite{}, the cost of the above operations is linear to the length $\ell$, however, our framework leverages data dependencies to perform multiple independent operations in a single round, reducing the total number of rounds to a logarithmic factor. \john{Check if ABY3 does this as well}
%We provide more details on this optimization in the APPENDIX.

\john{This could be moved in the background}
Special cases of the above primitive operations enable further optimizations. Less-than-zero checks ($s < 0$) require no communication between parties \cite{} \john{Is there a ref for that?} and can be used to reduce the number of rounds in equalities with public constants ($s = c$). In this case, instead of sharing the secret $s$ and do the general-purpose secure equality with the constant $c$, the data owners can first compute two subtractions $s-c$ and $c-s$ locally (in the clear) and share secrets of the results. This way, checking $s=c$ is reduced in two oblivious inequalities $s-c < 0$ and $c-s < 0$, both of which are local. This optimization exists in other MPC frameworks as well \cite{crypten} and we use it to evaluate selection predicates in SQL queries locally. %, as we explain later.

\stitle{Addition/Conversion.} Although oblivious addition using arithmetic shares is local (cf.~Section~\ref{sec:primitives}), oblivious addition using boolean shares requires $\ell$ rounds~\cite{}. The number of rounds can be reduced to $\mathcal{O}(\log\ell)$ using a parallel prefix adder, as in \cite{} \john{Add ref}, at the cost of exchanging more data between parties. 
%We provide more details on this in the APPENDIX. 
Oblivious addition using boolean shares is the main operation behind converting boolean shares to arithmetic and vice versa~\cite{}. \john{Add ref} %, and dominates the cost of these operations.%, as shown in Table~\ref{tab:primitive_costs}. 

One special case of conversion that is useful in many real queries is the boolean-to-arithmetic conversion of shares for single-bit secrets. This conversion can be done in two rounds using the protocol described in~\cite{} \john{Add ref}. In Section~\ref{sec:optimizations}, we explain how we leverage this optimization to speedup oblivious SQL aggregations.

\stitle{Compare-and-swap.} Finally, recall from Section~\ref{sec:primitives} that an oblivious compare-and-swap between $a$ and $b$ requires computing two formulas: $\texttt{min}~=~g\cdot b + (1-g)\cdot a$ and $\texttt{max}~=~g\cdot a + (1-g)\cdot b$, where $g$ is the result (0/1) of the inequality check $a > b$.  Evaluating these formulas requires $\lceil\log(\ell+1)\rceil$ rounds for the inequality plus two more rounds: one for exchanging $g$ shares and a second one to complete the multiplications.
}

\begin{table}[t]
\begin{center}
 \begin{tabular}{||c c c ||} 
 \hline
 Operator & \#operations & \#communication rounds \\ [0.5ex] 
 \hline\hline
\texttt{SELECT} &  $\mathcal{O}(n)$ & $\mathcal{O}(1)$   \\  % (\texttt{=}) 
  \hline
 \texttt{PROJECT} & $\mathcal{O}(n)$ & 0 \\
 \hline
\texttt{JOIN} & $\mathcal{O}(n\cdot m)$ &$\mathcal{O}(1)$  \\
 \hline
\texttt{SEMI-JOIN} & $\mathcal{O}(n\cdot m)$ & $\mathcal{O}(\log m)$  \\
 \hline
 \texttt{GROUP-BY} & $\mathcal{O}(n\cdot \log^2n)$ & $\mathcal{O}(n)$  \\
  \hline
 \texttt{ORDER-BY} & $\mathcal{O}(n\cdot \log^2n)$ & $\mathcal{O}(\log^2n)$  \\
 \hline
 \texttt{DISTINCT} & $\mathcal{O}(n\cdot \log^2n)$ & $\mathcal{O}(\log^2n)$  \\ [1ex]
 \hline
\end{tabular}
\caption{Summary of costs for oblivious relational operators \emph{w.r.t.} the cardinalities ($n$, $m$) of the input relation(s). JOIN is the most expensive operator in \#operations whereas GROUP-BY is the most expensive operator in \#rounds.}
 \label{tab:costs}
%These costs can be further reduced using oblivious hashing as described in Section~\ref{}.}
%The number of rounds required by \texttt{SELECT} and \texttt{JOIN} is independent of the input size.
\end{center}

\end{table}

\john{Should give the lower-bound of communication rounds in Table 1 and talk about batching? For communication, these are actually lower-bounds, not upper bounds.}

\subsection{Relational operators}\label{sec:cost_relational}
 
We now analyze the costs of relational operators. Let $R$, $S$ be relations of size $n$ and $m$ respectively (number of rows). Table~\ref{tab:costs} shows the number of operations as well as the communication rounds required by each individual operator with respect to the input size.  %In the following, we denote an attribute $$ $R.a$, $S.b$ be the attributes $a$ and $b$ in $R$ and $S$

\stitle{PROJECT.} Oblivious \texttt{PROJECT} is as cheap as its cleartext counterpart: it requires $n$ local operations and zero communication rounds, as each party simply discards the shares that correspond to the filtered attributes. Oblivious 

\stitle{SELECT.} Oblivious \texttt{SELECT} needs to traverse the whole input relation, let $R$, however, the number of communication rounds is independent of $R$'s size ($|R|=n$) and only depends on the selection predicate. For instance, if the selection predicate includes a single equality (e.g. $R.a = c$, where $c$ is a public constant, the equality check can be reduced into two local less-than-zero checks (cf. Section~\ref{sec:cost_primitives}). On the other hand, if the selection predicate involves an inequality (e.g. $R.a > c$), the number of required rounds is $\lceil\log(\ell+1)\rceil$. 
Regardless of the actual predicate, all $n$ predicate applications in \texttt{SELECT} do not depend on each other and, thus, they can be evaluated \emph{in bulk} for an arbitrary number of rows $k$, $k\leq n$. In a bulk evaluation, each one of the  rounds required by the selection predicate is performed with a \emph{single} data exchange for \emph{all} rows together. This way, the total number of rounds (i.e. synchronization barriers) required by \texttt{SELECT} equals the total number of rounds required to evaluate the selection predicate on a \emph{single} row. 

\stitle{JOIN.} Oblivious \texttt{JOIN}  is the most expensive operation in terms of CPU cost as it requires a nested-loop over the input relations to check all possible pairs ($n\cdot m$); however, the number of communication rounds in the oblivious \texttt{JOIN} is independent of the input sizes $n$ and $m$. As in the case of \texttt{SELECT}, the number of rounds only depends on the join predicate. For equality joins, each one of the $n\cdot m$ equality checks requires $\lceil\log\ell\rceil$ rounds (where $\ell$ is the length of the join attributes in bits) and is independent of others, hence, the whole join can be done in $\lceil\log\ell\rceil$ rounds. Range joins are more expensive. A range join with predicate of the form $R.a \leq S.b$, where $a$, $b$ are attributes of the input relations $R$ and $S$, requires $\lceil\log(\ell+1)\rceil$ rounds in total. The constant asymptotic complexity with respect to the input size holds for \emph{any} $\theta$-join. % and this is a nice property we leverage in our framework to speedup join queries.
%We analyze more complex $\theta$-joins in Section~\ref{}.

\stitle{SEMI-JOIN.} Oblivious semi-joins require the same number of operations as the $\theta$-joins but the number of communication rounds is different. A semi-join $R\ltimes_\theta S$ requires $\mathcal{O}(\log|S|)$ communication rounds to evaluate the formula $\bigvee_{\forall t'\in S}\theta(t, t')\}$ from Section~\ref{sec:secure_operators}. This formula requires ORing $|S|$ bits, which can be done in $\lceil\log|S|\rceil$ communication rounds by using a binary tree of logical operators, as in the case of equality and inequality (cf. Section~\ref{primitives}).  \john{I think we need to say this early in the background.} % and doing the evaluation in a bottom-up fashion. 

\stitle{ORDER-BY.} Oblivious \texttt{ORDER-BY} relies on Bitonic sort that performs $\mathcal{O}(n\cdot\log^2n)$ compare-and-swap operations in $\frac{\log n(1 + \log n)}{2}$ stages, where each stage involves $\frac{n}{2}$ independent compare-and-swap operations that can be performed in bulk. Given the I/O cost of compare-and-swap operations from Section~\ref{sec:cost_primitives}, the total number of rounds required by \texttt{ORDER-BY} is:

\[
  \frac{\log n\cdot(1 + \log n)}{2} \cdot \Bigg(\Big\lceil\log(\ell+1)\Big\rceil +2\Bigg) %= \mathcal{O}(\log^2n)
 \]

\noindent
where $n$ is the cardinality\footnote{Oblivious sorting algorithms require $n$ to be a power of two, thus, the data owners must pad their data accordingly before sending secret shares to computing parties.} of the input relation, and $\ell$ is the length of the sort attribute in bits. The analysis assumes one sorting attribute. Adding more sorting attributes increases the number of rounds in each comparison by a small constant factor. %, so the asymptotic complexity remains the same.
 
\stitle{DISTINCT.} Oblivious \texttt{DISTINCT} and \texttt{GROUP-BY} require the same asymptotic number of operations as \texttt{ORDER-BY}. This is because their CPU cost is dominated by their first phase that includes sorting (cf. Section~\ref{sec:operator_impl}). 
\texttt{DISTINCT}'s communication cost is also dominated by that of \texttt{ORDER-BY}.
%is only slightly more expensive in terms of communication rounds. 
In the second phase of \texttt{DISTINCT}, the operator scans the sorted input relation and compares each pair of adjacent rows on the distinct attribute ($n-1$ pairs in total). 
%The \texttt{DISTINCT} operator breaks in two phases: in the first phase, it requires sorting the relation on the attribute in the \texttt{DISTINCT} clause, let $a$, whereas, in the second phase, it scans the sorted relation $R$ and compares each pair of adjacent rows on $a$ ($n-1$ pairs in total). 
This step requires only $\lceil\log\ell\rceil$ rounds since all $n-1$ equality checks are independent from each other and can be performed in bulk. Thus, the total number of rounds in oblivious \texttt{DISTINCT} is:

\[
  \frac{\log n\cdot(1 + \log n)}{2} \cdot \Bigg(\Big\lceil\log(\ell+1)\Big\rceil +2\Bigg) + \Big\lceil\log\ell\Big\rceil
 \]

\noindent
where n is the cardinality of the input relation, and $\ell$ is the length of the \texttt{DISTINCT} attribute in number of bits.

\stitle{GROUP-BY.} The most expensive operator in terms of communication rounds is \texttt{GROUP-BY} with aggregation.  After the initial sorting phase (on the group-by key), the operator scans the input and applies the aggregation function \emph{sequentially}, that is, each aggregation step requires synchronous communication between parties before proceeding to the next tuple. In the end, the  operator performs a final shuffling, which has the same cost as an oblivious sorting, hence, 
%which breaks into the following three phases. First, it  sorts the input relation on the \texttt{GROUP-BY} attribute. Second, it scans the sorted relation and applies the aggregation function e.g. \texttt{AVG}, \texttt{COUNT}, etc., on each pair of adjacent rows ($n-1$ pairs in total). The aggregation has to be applied sequentially, that is, to proceed to the next pair, the operator must first finish all rounds of the evaluation on the current pair. In the third phase, \texttt{GROUP-BY} requires one oblivious suffling to hide the group boundaries when opening the relations to the learner\footnote{ In the context of SQL queries, the third phase can be omitted if the \texttt{GROUP-BY} is followed by another sort-based operator, i.e,. \texttt{ORDER-BY} or \texttt{DISTINCT}.}. Oblivious suffling is essentially oblivious sorting~\cite{}, 
the total number of rounds required by \texttt{GROUP-BY} is: 

\[
  %\log n\cdot(1 + \log n) \cdot \Bigg(\Big\lceil\log(\ell+1)\Big\rceil +2\Bigg) + (n-1)\cdot  \Bigg(\Big\lceil\log\ell\Big\rceil + r_{agg}\Bigg) 
  \log n\cdot(1 + \log n) \cdot \Bigg(\Big\lceil\log(\ell+1)\Big\rceil +2\Bigg) + (n-1)\cdot  c_{agg}
 \]
 
 \noindent
where $n$ is the cardinality of the input relation, $\ell$ is the length of the \texttt{GROUP-BY} key in bits, and $c_{agg}$ is the number of rounds required to apply the aggregation function to a pair of rows (independent of the input size $n$). 
%The aggregations we support are \texttt{AVG}, \texttt{COUNT}, \texttt{SUM}, \texttt{MIN}, and \texttt{MAX}. Details on $c_{agg}$ for each function are given in the APPENDIX.
When applied to big relations, oblivious \texttt{GROUP-BY} can incur a prohibitive number of rounds (linear to the relation size), although the amount of data exchanged at each round is small. The high communication cost of \texttt{GROUP-BY} can be significantly reduced using oblivious hashing. We discuss this optimization in Section~\ref{sec:next}.

\stitle{Aggregations.} Aggregations in SQL can be used without a \texttt{GROUP-BY} clause. In this case, applying the aggregation function requires $n-1$ operations in total but the number of communication rounds is reduced from $\mathcal{O}(n)$ (when combined with a \texttt{GROUP-BY} clause) to $\mathcal{O}(\log n)$. To achieve this, we have to build a binary tree of operations whose leaves correspond to the $n$ rows of the input relation and do the evaluation bottom-up. At each tree level $k\geq1$, we apply all independent $\frac{n}{2^k}$ aggregations within a single communication round, and we continue with the next level until we reach the root of the tree. This optimization makes aggregations efficient in practice. It can also been used to reduce the number of rounds in \texttt{GROUP-BY} to a logarithmic factor, provided that the data owners agree to reveal the group sizes  \cite{cryptoeprint:2020:599, DBLP:journals/iacr/IonKNPRSSSY19}. \john{Are these references correct?}

%\begin{table}[t]\small
%\begin{center}
% \begin{tabular}{||c c c ||} 
% \hline
% \multirow{2}{*}{Operator} & \#comm. rounds  & \#comm. rounds 
% & & (\textttt{GROUP-BY}) &  (plain)\\ [0.5ex]
% \hline\hline
% \texttt{AVG} &$\mathcal{O}(1)$  & \\
%% \hline
%% Range-Join & $n\cdot m$ & $\mathcal{O}(1)$  \\
% \hline
%\texttt{COUNT/SUM}  & $(n-1)\cdot(5+\lceil\log\ell\rceil)$  &  $\log n \cdot(5+\lceil\log\ell\rceil)$\\  % (\texttt{=}) 
%  \hline
% %\texttt{SUM} & $n-1$ & $(n-1)\cdot(4+\log\ell)$ & $\log n \cdot(4+\log\ell)$\\
%% \hline
% \texttt{MIN/MAX}  & $(n-1)\cdot(3+\lceil\log\ell\rceil)$  & $\log n\cdot(3+\lceil\log\ell\rceil)$ \\  [1ex]
% \hline
%\end{tabular}
%\caption{Summary of costs for aggregation functions supported by our framework. All aggregations perform $n-1$ operations, where $n$ is the cardinality of the input, but they have different costs in terms of communication rounds.} 
% \label{tab:costs}
%%These costs can be further reduced using oblivious hashing as described in Section~\ref{}.}
%%The number of rounds required by \texttt{SELECT} and \texttt{JOIN} is independent of the input size.
%\end{center}
%
%\end{table}

%\vasia{Discuss the trade-off between the number of communication rounds and the data amplification (memory requirements) for each operator. We need to explain batching and provide a cost analysis that takes into account the batch number and size.}

\stitle{Cost of composition.}
As mentioned in Section~\ref{sec:constructing_plans}, composing oblivious operators incurs additional communication cost.
For example, consider a query $\sigma_{R.a=c}(R)\bowtie_{R.b=S.d}S$ between two relations $R(a,b)$ and $S(d,e)$.
%\begin{verbatim}
%SELECT e 
%FROM R, S
%WHERE R.a = c AND R.b = S.d
%\end{verbatim}\vspace{1mm}
This query involves two operators, namely a selection and a join. Let $\ell$ be the length of all attributes $a$, $b$, $c$, and $d$. According to the cost analysis above, both the selection and the join require $\lceil\log\ell\rceil$ rounds each to evaluate the equality predicates. 
Composing these two operators in a plan results in $2\cdot\lceil\log\ell\rceil + 1$ rounds of communication in total. In this example, there is only one additional round because the logical AND between the results of the two predicates can be done in bulk. In other cases, however, composition of operators can incur a high communication cost. In the example of Section~\ref{sec:constructing_plans}, the logical AND of the three bits (line \textbf{4} in Algorithm~\ref{alg:composite_group}) incurs two additional rounds at each step of the for loop. Communication overheads due to composition of operators depend on the actual query. 

\john{I realized that the query above can in fact be evaluated in $\lceil\log\ell\rceil$ rounds, since all equality checks are independent from each other..} 


\subsection{Data overhead of oblivious operations}\label{sec:data_overhead}

We now quantify the overhead of oblivious operations with respect to the amount of data they need to exchange.
Equality checks ($=, <>$) and boolean addition require exchanging  $p\cdot(\ell - 1)$ bits, where $p$ is the number of parties (in our case 3) and $\ell$ is the length of the elements being compared or added (in number of bits). For instance, if we want to compare two 64-bit integers, the computing parties need to exchange $3 \cdot 63 = 189$ bits $\approx 24$ bytes in total (in $\log64 = 6$ rounds). Inequality checks are more expensive and require exchanging $\sim120$ bytes in total (in $\lceil\log65\rceil = 7$ rounds). \john{We might to say why e.g. because inequality requires evaluating a more complex formula.. We can simply say something in the background and just refer to the background section.}
%Lastly, boolean addition of $\ell$-sized numbers in $\ell$ rounds has the same cost with equality.

We can estimate the amount of data exchanged during the evaluation of oblivious relational operators using the number of operations in Table~\ref{tab:costs} and the data exchanged by each primitive involved in the operator. 
For instance, a simple \texttt{GROUP-BY} operator with a \texttt{SUM} on a relation with two 64-bit attributes and $10K$ rows requires exchanging $\sim 320MB$ in total, most of which are needed to sort the relation on the \texttt{GROUP-BY} key and shuffle it in the end (the actual aggregation generates only a few $MBs$).
The most expensive operator in terms of data exchanged between parties is the \texttt{JOIN}, as it involves a high number of operations. For example, joining two relations with $10K$ rows each on a common 64-bit attribute requires exchanging $\sim2.4GB$. A range-join between the same two relations would require $\sim12GB$. \john{CHECK ESTIMATIONS}

%This is a considerable overhead which we can reduce via oblivious hashing, as we explain in the next section.
 
%\john{We need a table that summarizes the formulas to estimate size of data exchanged during each operator. We also need to distinguish between the overhead of intermediate data maintained by each party (vs communication rounds) and the overhead of data sent over the wire.}


==> framework.tex <==




==> oblivious.tex <==
\subsection{Oblivious operator implementation}\label{sec:operator_impl}

Our oblivious operators do not only hide their output size but also the access patterns they perform. One way to `hide'  access patterns is to implement the operator in a way that makes its control-flow independent of the input data so that it incurs exactly the same accesses for all inputs of the same size. In practice, this means that the implementation does not include any \texttt{if} statements that depend either directly or indirectly on the input data.

Implementing the oblivious selection, join, and semi-join is straight-forward. Selection requires a simple scan over the input relation, while join and semi-join require a nested-loop over the two inputs. In all cases, the operator's predicate is evaluated under MPC using the primitives of Section~\ref{sec:secure_primitives}. 
%, and the result is stored at the extra attribute introduced.

%Group-by, distinct, and order-by operators require more careful implementation.

Group-by and distinct operators are based on oblivious order-by, which is typically implemented using a bitonic sorter, such as Batcher's sort~\cite{10.5555/280635}. Bitonic sort has data-independent control flow and performs $\mathcal{O}(n\log^2n)$ comparisons, where $n$ is the cardinality of the input. Our oblivious order-by operator implements Batcher's sort control flow and orders tuples using oblivious compare-and-swap operations (cf. Section~\ref{sec:secure_primitives}).
%, and its control flow (the elements being compare at each step of the algorithm) does not depend on the result of previous steps, as in other sorting algorithms (e.g. quick-sort). 

The logic of oblivious group-by is given in Algorithm 1 and is based on the protocol in~\cite{DBLP:journals/iacr/JonssonKU11}.   
Let $a_k$ be the group-by key, $a_w$ the aggregated attribute, and $a_g$ the extra attribute that stores the aggregation result (same notation as in Section~\ref{sec:secure_operators}).  The first step is to sort the input relation on the group-by key (\textbf{line 1}). Then, the operator scans the sorted relation and, for each pair of adjacent tuples, applies an oblivious equality comparison on $a_k$  (\textbf{line 3}). The result of this comparison ($b$) is used to aggregate (\textbf{line 4}) and `mask' (\textbf{lines 5-7}) obliviously. Aggregation is updated incrementally based on the values of the last pair of tuples. \texttt{MIN}, \texttt{MAX}, \texttt{COUNT}, and \texttt{SUM} can be easily evaluated this way but for \text{AVG} we need to keep the sum (numerator) and count (denominator) separate.

When the scan is over, the algorithm requires a final shuffling to hide the group `traces' in case the relation (or a part of it) is opened to the learner(s). Oblivious shuffling is essentially oblivious sorting: each party appends a new attribute to $R$, which is populated with locally generated random values, and sorts $R$ on this attribute. After shuffling, the extra attribute can be discarded. In the context of multi-operator queries, the final shuffling is needed only if there is no subsequent order-by in the query plan, which would obliviously re-order $R$ anyway.

\begin{algorithm}[t]
\small
%\Input{A stream $S$ of logs and a window $[t_s,t_e]$;}
%\Output{The graph snapshot $G_{[t_s,t_e]}$;}

%\BlankLine

%\Comment{The sort direction does not matter}
sort input relation R on $a_k$;

%let $a_k$ be the group-by key, $a_w$ the aggregated attribute, and $a_g$ the extra attribute that stores the aggregation result;

\For {each pair of adjacent tuples ($t_i$, $t_{i+1}$), $0\leq i < |R|$,} {
  
  \Comment{Are tuples in the same group?}
  
  let $b \leftarrow t_i[a_k] \stackrel{?}{=} t_{i+1}[a_k]$;
  
  \Comment{Aggregation}
  
  $t_{i+1}[a_g] \leftarrow b\cdot agg\Big(t_i[a_w], t_{i+1}[a_w]\Big) + (1-b)\cdot t_{i+1}[a_g]$;
  
  \Comment{Masking}
  \For {each attribute $a$ of $t_i$} {
  	
	let $r$ a random value;
	
  	$a \leftarrow b\cdot r~~+~~(1-b)\cdot a$;
  } 
  
  shuffle R; %\Com{Only if there is no subsequent order-by}
}


%re-distribute $E_h$ based on $(id_{src},id_{dst},id_{corr})$;
%Pair up half edges in each partition and create the set $E_{comm}$ of edges for communication activities;
%\textbf{return} $E_w \cup E_{c}$
\caption{\small Main control-flow of oblivious group-by}\label{alg:group}
\end{algorithm}

Distinct is a special case of group-by and has a similar but simpler logic. The first step of distinct is to sort the input relation on $a_k$ (in this case the distinct attribute), as in Algorithm~\ref{alg:group}. Then, the operator scans the sorted relation and, for each pair of adjacent tuples, it applies the equality comparison on $a_k$ (\textbf{line 3}) and sets the distinct bit $t_{i+1}[a_g]$ to $\lnot b$ (the value $t_0[a_g]$ of the first tuple is set to 1). The distinct operator does not require masking or shuffling, hence, lines \textbf{5-8} in Algorithm~\ref{alg:group} are simply omitted for distinct.

Although group-by and distinct have similar logic, their communication costs are quite different: in group-by, the value  $t_{i+1}[a_g]$ (\textbf{line 4}) depends on the result of the previous aggregation (as it depends on $t_{i}[a_g]$) whereas, in distinct, setting the bit $t_{i+1}[a_g]$ to $\lnot b$ does not depend on the previous step of the for-loop. This enables parties to communicate asynchronously, which in turn makes the distinct operator more efficient in practice than group-by. We analyze all operator costs in Section~\ref{sec:costs}.

\john{Say something about this in the implementation section: A secure framework would always require formal verification to make sure that no information is leaked (e.g. due to bugs). Formally verifying the end-to-end obliviousness of our implementation is out of the scope of this paper and we leave it for future work. }

%\begin{algorithm}[t]
%\small
%%\caption{\small Oblivious Group-by}\label{alg:pag}
%%\Input{A stream $S$ of logs and a window $[t_s,t_e]$;}
%%\Output{The graph snapshot $G_{[t_s,t_e]}$;}
%
%%\BlankLine
%
%sort input relation R on $a_k$;
%
%$t_{0}[a_g] \leftarrow 1$;
%
%\For {each pair of adjacent tuples ($t_i$, $t_{i+1}$) in $R$} {
%  
%  let $b \leftarrow t_i[a_k] \stackrel{?}{=} t_{i+1}[a_k]$;
%  
%  \Comment{Set distinct bit}
%  
%  $t_{i+1}[a_g] \leftarrow b$;
%  
%}
%%re-distribute $E_h$ based on $(id_{src},id_{dst},id_{corr})$;
%%Pair up half edges in each partition and create the set $E_{comm}$ of edges for communication activities;
%%\textbf{return} $E_w \cup E_{c}$
%\end{algorithm}



==> operators.tex <==
\section{Relational MPC}\label{sec:framework}
\subsection{Oblivious relational operators}\label{sec:secure_operators}

\john{Say something about queries in MPC (aggregations) in contrast to queries in standard db benchmarks}

%In this work, we focus on queries with aggregations and joins that do not reveal any of the original input data. For example, we assume that any column appearing in the \texttt{SELECT} also appears in a \texttt{GROUP BY} clause. We make no restriction either on the number of input relations or on the number of joins among them. We also consider queries with \texttt{DISTINCT}, \texttt{LIMIT}, and \texttt{ORDER BY}.
%In summary, we consider SQL queries of the
%following form.
%%form shown in Figure \ref{fig:sql-format}.
%
%
%% \begin{figure}[h]
%\begin{verbatim}
%SELECT [ ALL | DISTINCT ]  
%    [ agg_fun (ALL | DISTINCT expression) ]
%    [ column_name | expression ]
%FROM [ table_name [ ,...n ] ]
%WHERE [...]
%GROUP BY [column_name [,...n] ]
%ORDER BY [... [,...n] ]
%LIMIT k 
%\end{verbatim}
%% \caption{Supported class of SQL queries\label{fig:sql-format}}
%% \end{figure}

%\vasia{Categorize operators as follows: (1) Column-appending (select, semi-join, distinct, group-by), (2) In-place (order-by), (3) expanding (amplifying) i.e. join.}

%\john{We need one figure depicting what each operator is doing.}

In this section, we define the oblivious operators used in our framework.
Let $R$, $S$, and $T$ be three relations with cardinalities $|R|$, $|S|$, and $|T|$ respectively. Let also $t[a_i]$ be the value of attribute $a_i$ in tuple $t$. To simplify the presentation, we define operators as if the relations they are applied to and the relations they define are \emph{opened} (cf. Section~\ref{}). Specifically, when we say that an operator is applied to a relation $R$ and defines another relation $T$, this means that each computing party has \emph{shares} of $R$ and $T$, that is, $\llbracket R\rrbracket$  and $\llbracket T\rrbracket$.

%= T_{\llbracket a_1\rrbracket, \llbracket a_2\rrbracket, ..., \llbracket a_m\rrbracket}$.

\stitle{PROJECTION.} Oblivious projection has the same semantics as the non-oblivious operation: 

\[
\prod_{A}{(R)} = R_A
\]\vspace{1mm}

\noindent
where $A$ is a list of attribute names from $R$. Projection has no additional overhead under MPC and can be done locally by each party (without communication), as in a clear-text evaluation.

\stitle{SELECTION.}
An oblivious selection with predicate $\varphi$ on a relation $R$ defines a new relation:

\[
 T= \{t\cup\{\varphi(t)\}~~|~~t\in R\}\\ \\
\]\vspace{0.5mm}

%\[
%\sigma_{\varphi}(R) = R'_{a_1, a_2, a_3, ..., a_m, a_{m+1}}
%\]\vspace{1mm}

\noindent
 with the same cardinality as $R$, i.e. $|T|=|R|$, and one more attribute for each tuple $t\in R$ that contains $\phi$'s result when applied to $t$ (each party has shares of this result). The result is a single bit (0/1) denoting whether the tuple $t$ is included in $T$ (1) or not (0). The predicate $\phi$ can be an arbitrary logical expression with atoms that may also include arithmetic expressions ($+,*, =, >, <, \neq, \geq, \leq$). Such expressions are evaluated under MPC using the primitives of Section~\ref{}. Note that, in contrast to a typical selection in the clear, oblivious selection defines a relation with the same cardinality as the input relation, i.e., it does not remove tuples from the input so that the size of the output remains hidden to the computing parties.
 
\stitle{JOIN.}  An oblivious $\theta$-join between two relations $R$ and $S$, denoted with $R\bowtie_\theta S$, defines a new relation:

\[
 T = \{(t\cup t'\cup\{\theta(t, t') \})~~|~~t\in R~\wedge~t'\in S\}\\ \\
\]\vspace{0.5mm}

\noindent
where $t\cup t'$ is a new tuple that contains all attributes of $t\in R$ along with all attributes of $t'\in S$, and $\theta(t, t')$ is $\theta$'s result when applied to the pair of tuples ($t, t'$). This result is a single bit (0/1) denoting whether the tuple $t$ `matches' with tuple  $t'$ (1) or not (0) according to $\theta$. As in the case of selections, the join predicate can be an arbitrary logical expression with atoms that may also include arithmetic expressions.

Intuitively, an oblivious $\theta$-join generates the cartesian product of the input relations ($R\times S$), where each tuple is augmented with an additional attribute that stores the result share of applying the join predicate to the corresponding pair of input tuples. Join is the only oblivious operator in our framework that generates a relation with cardinality larger than the cardinalities of its inputs.  

\stitle{SEMI-JOIN.} An oblivious (left) semi-join between two relations $R$ and $S$ on a predicate $\theta$, denoted with $R\ltimes_{\theta}S$, defines a new relation:

\[
 T = \{(t\cup\{\bigvee_{\forall t'\in S}\theta(t, t')\})~~|~~t\in R\}\\ \\
\]\vspace{0.5mm}

\noindent
with the same cardinality as $R$, i.e. $|T|=|R|$, and one more attribute that stores the result of the formula 
$\bigvee_{\forall t'\in S}\theta(t, t')$. The latter denotes the logical OR of the $|S|$ bits produced by applying $\theta$ to $|S|$ pairs of tuples.
% ($|S|$ bits for each tuple $t\in R$).   

%Let $b = t_i[a_k]\geq t_j[a_k]$ be the result (0/1) of the inequality comparison between attribute values $t_i[a_k]$ and $t_j[a_k]$. An oblivious compare-and-swap between indices $i, j$ requires computing the following two formulas under MPC:
%
%\[
%i \leftarrow b\cdot j~+~(1-b)\cdot i
%\]
%\[
%j \leftarrow b\cdot i~+~(1-b)\cdot j
%\]\vspace{1mm}
%
%Oblivious compare-and-swap updates the values $i, j$ in-place.
%%initially, each tuple $t$ assigned a unique index $i$, $1\leq i\leq|R|$, that defines a random order in $R$. 
%Note that each party computes the above formulas using the respective shares and, hence, cannot identify the new `multiplexed' values of $i$ and $j$.

\stitle{GROUP-BY with aggregation.} An oblivious group-by aggregation on a relation $R$ with $m$ attributes defines a new relation $T=\{f(t')~~|~~t'=t\cup\{a_{g}\},~~t\in R\}$ with the same cardinality as $R$, i.e. $|T|=|R|$, and one more attribute $a_{g}$ that stores the result of the aggregation.
Let $a_k$ be the group-by key and $a_w$ the attribute whose values are aggregated. Let also $S = \Big[t_1[a_w], t_2[a_w], ..., t_u[a_w]\Big]$ be the list of values for attribute $a_w$ for all tuples $t_1, t_2, ..., t_u\in R$ that belong to the same group, i.e.,   $t_1[a_w]=t_2[a_w]=...=t_u[a_w]$, $1\leq u\leq |R|$. The function $f$ in $T$'s definition above is defined as follows:

\[
    f(t_i)=\left\{
                \begin{array}{ll}
                  t_i[a_{g}] = agg(S),~~i=v,~~1\leq v\leq u\\ \\
                  t_{random},~~i\neq v,~~1\leq i\leq u\\ 
                \end{array}
              \right.
\]\vspace{1mm}

\noindent
where $t_{random}$ is a tuple whose first $m$ attributes are randomly generated whereas the last one ($a_g$) is set to an  invalid aggregation result (e.g. the maximum possible value). The function $agg(S)$ is the aggregation function, e.g. \texttt{MIN}, \texttt{MAX}, \texttt{COUNT}, \texttt{SUM}, \texttt{AVG}. Aggregation functions are computed using the primitives of Section~\ref{}.

In simple words, oblivious aggregation sets the value of $a_g$ in one tuple per group equal to the result of the aggregation for that group and updates (in-place) all other tuples with `garbage'.
Groups can be defined on multiple attributes (keys) using the standard semantics. Oblivious aggregation on an attribute of a relation $R$ (without a group-by) is defined as before, assuming that all tuples in $R$ belong to the same group.

\stitle{DISTINCT.} The oblivious distinct operator is a special case of group-by with aggregation, assuming that $a_k$ is not the group-by key as before but the attribute where distinct is applied. For distinct, the function $f$ is defined as follows:

\[
    f(t_i)=\left\{
                \begin{array}{ll}
                  t_i[a_{g}]=1,~~i=v,~~1\leq v\leq u\\ \\
                  t_i[a_{g}]=0,~~i\neq v,~~1\leq i\leq u\\
                \end{array}
              \right.
 \]\vspace{0.5mm}

\stitle{ORDER-BY.} %Oblivious sorting has the same semantics as the non-oblivious operation. 
Sorting a relation $R$ with $m$ attributes on ascending (resp. descending) order of an attribute $a_k, 1\leq k\leq m$, results in a new relation $s_{\uparrow a_k}(R) = T$ (resp. $s_{\downarrow a_k}(R) = T$), where each tuple is assigned an index $i$ such that:

 \[
    \forall t_i, t_j \in R, i < j \iff \left\{
                \begin{array}{ll}
                   t_i[a_k] < t_j[a_k]~~~(\texttt{ASC})\\ \\
                   t_i[a_k] > t_j[a_k]~~~ (\texttt{DESC})\\
                \end{array}
              \right.
 \]\vspace{0.5mm}

Sorting has the same semantics with its non-oblivious counterpart, however, the tuple ordering is computed under MPC using oblivious compare-and-swap operations (cf. Section~\ref{}). 
We can define sorting on multiple attributes using the standard semantics. For example, sorting a relation $R$ first on attribute $a_i$ (ascending) and then on $a_j$ (descending) is denoted as $s_{\uparrow a_i \downarrow a_j}(R)$.

An order-by operator is often followed by a limit that defines the number of tuples the operator must output. Limit in the oblivious setting has the same semantics. Order-by with limit is the only operator in our framework that may output a relation with cardinality smaller than the cardinality of its input.

\stitle{MASK.} Multiplexing in case of non-aggregated results. \john{TODO} In 

\stitle{Remark.} All operators we define, except \texttt{PROJECT} and \texttt{ORDER-BY}, introduce a new attribute that stores the result of a logical or arithmetic expression evaluated under MPC. For example, selection introduces an attribute that stores the result of the selection predicate applied to each tuple, whereas group-by uses an extra attribute to store the result of the aggregation.
The purpose of this extra attribute (along with the additional `masking' of tuples in group-by) is to hide the actual output size from the computing parties. This way, the parties can jointly compute the output of an operator without identifying, e.g., how many tuples are filtered out by the selection, how many tuples match the join predicate or how many groups exist in a relation. The tuples that are actually included in an operator's output are identified by this extra attribute whose value is computed under MPC and shared amongst parties. Even if an operator is the final one in a query plan, its result set and actual size are only revealed to the \emph{learner(s)} (cf. Section~\ref{}) when the computation is over.



==> queries.tex <==
\subsection{Optimizations on real queries}\label{sec:queries}

  \begin{figure}[t]
    \centering
        \begin{minipage}{.14\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/drawings/comorbidity-plan.png}
            \vspace{-6mm}
            \caption{Comorbidity}\label{fig:comorbidity-plan}
            \end{subfigure}
        \end{minipage}
        \begin{minipage}{.18\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/drawings/cdiff-plan.png}
            \vspace{-6mm}
            \caption{Recurrent C.Diff.}\label{fig:cdiff-plan}
            \end{subfigure}
        \end{minipage}
              \begin{minipage}{.24\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/drawings/aspirin-plan.png}
            \vspace{-6mm}
            \caption{Aspirin Count}\label{fig:cdiff-plan}
            \end{subfigure}
        \end{minipage}
        \caption{Optimized query plans for three real queries}\label{fig:opt-plans}
    \end{figure} 


We now showcase the applicability of \ours's optimizations on three queries from clinical studies~\cite{pcornet, pcori, clostridium} that have also been used in other MPC works~\cite{Bater2017SMCQL,Volgushev2019Conclave,bater2018shrinkwrap,bater2020saqe,Poddar2021Senate}. 
We experimentally evaluate the performance benefits on a larger set of queries in Section~\ref{sec:evaluation}.

%\vasia{baseline plans found there}. 

\stitle{Comorbidity.} This query returns the ten most common diagnoses of individuals in a cohort. 
%t includes a semi-join between \texttt{diagnosis} and \texttt{cdiff\_cohort} followed by \texttt{GROUP-BY} and an \texttt{ORDER-BY} on an intermediate attribute (\texttt{cnt}). 
\vspace{1mm}
%This query includes a \texttt{LIMIT} clause that we can use to showcase the \texttt{ORDER-BY} optimization with \texttt{LIMIT}), although this exists in previous works as well.

{\small 
\texttt{SELECT diag, COUNT(*) cnt}

\texttt{FROM diagnosis}

\texttt{WHERE pid IN cdiff\_cohort}

\texttt{GROUP BY diag}

\texttt{ORDER BY cnt DESC}

\texttt{LIMIT 10}
}\vspace{1mm}

\noindent This query lends itself to join-aggregation decomposition and dual sharing, producing the plan shown in Figure~\ref{fig:opt-plans}a. Let $n$ be the cardinality of \texttt{diagnosis}. The number of operations needed to evaluate this query is $\mathcal{O}(n\log^2 n)$ (due to oblivious sorting) whereas the number of communication rounds is $\mathcal{O}(n)$ (due to the oblivious group-by). %,  where $n$ is the cardinality of \texttt{diagnosis}. 
The space requirements are bounded by the size of \texttt{diagnosis}, i.e., $\mathcal{O}(n)$.

\stitle{Recurrent Clostridium Difficile.} This query returns the distinct ids of patients who have been diagnosed with \texttt{cdiff} and have two consecutive infections between 15 and 56 days apart. \vspace{1mm}

%and uses the \texttt{PARTITION BY} clause to order records per patient on ascending order of \texttt{time}. The output of this subquery is then joined with itself using a complex predicate to identify the distinct ids of recurring patients . 

% that computes the distinct ids of patients whose infections fall in the specified time window. 
%In this case, we leverage the fact that the self-join of \texttt{rcd} checks adjacent records of the same patient and we use an optimization similar to the one described in Section~\ref{sec:fusion}. The only difference is that we evaluate the inequality predicates along with \texttt{DISTINCT}. 
{\small
\texttt{WITH rcd AS (}

\hspace{5mm}\texttt{SELECT pid, time, row\_no() OVER}
        
\hspace{5mm}\texttt{(PARTITION BY pid ORDER BY time)}

\hspace{5mm}\texttt{FROM diagnosis}
    
\hspace{5mm}\texttt{WHERE diag=cdiff)}

\hspace{2mm}\texttt{SELECT DISTINCT pid}

\hspace{2mm}\texttt{FROM rcd r1 JOIN rcd r2 ON r1.pid = r2.pid} 

\hspace{2mm}\texttt{WHERE r2.time - r1.time >= 15 DAYS}

\hspace{2mm}\texttt{AND r2.time - r1.time <= 56 DAYS}

\hspace{2mm}\texttt{AND r2.row\_no = r1.row\_no + 1}
}\vspace{1mm}

\noindent Two optimization are applicable in this case. First, we apply blocking operator push-down to sort on \texttt{diagnosis} before applying the selection. Second, we use distinct fusion ($\sigma$-$\delta$) to evaluate the inequality predicates along with \texttt{DISTINCT}.
The optimized plan is shown in Figure~\ref{fig:opt-plans}b and it  requires $\mathcal{O}(n\log^2 n)$ operations and $\mathcal{O}(\log^2 n)$ communication rounds.
%, both due to oblivious sorting. The space requirements are again bounded by the size of \texttt{diagnosis}, that is, $\mathcal{O}(n)$. 
Note that an end-to-end oblivious implementation of the plan used in \cite{Bater2017SMCQL} requires
% $\mathcal{O}(n^2)$ space, 
 $\mathcal{O}(n^2\log^2 n)$ operations and $4\times$ more communication rounds, i.e., $\mathcal{O}(\log^2 n^2) = \mathcal{O}(4\log^2n) = \mathcal{O}(\log^2n)$. This is because \texttt{PARTITION BY} is not possible under MPC without revealing the number of partitions and, thus, the self-join will generate and materialize the cartesian product $\texttt{rcd}\times\texttt{rcd}$, before applying the final \texttt{DISTINCT} operation. %Materializing the cartesian product increases the space requirements to $\mathcal{O}(n^2)$. %By pushing \texttt{DISTINCT} before the join, we are able to pipeline the latter and keep the memory footprint bounded. We come back to this in Section~\ref{sec:implementation}.
 
\stitle{Aspirin Count.} The third query returns the number of patients who have been diagnosed with heart disease and have been prescribed \texttt{aspirin} after the diagnosis was made. \vspace{1mm}

{\small 

\texttt{SELECT count(DISTINCT pid)}

\texttt{FROM diagnosis as d, medication as m on d.pid = m.pid}

\texttt{WHERE d.diag = hd AND m.med = aspirin}

\texttt{AND d.time <= m.time}
}\vspace{1mm}

\noindent Here, we use blocking operator push-down and join push-up. We push the blocking distinct operator after the join to avoid materializing and sorting the join output. The optimized plan is shown in Figure~\ref{fig:opt-plans}c. 
% the optimization of Section~\ref{sec:push_down_blocking}, i.e., it pushes the blocking \texttt{DISTINCT} operator after the join between \texttt{diagnosis} and \texttt{medication} to avoid materializing and sorting the join output.
Let \texttt{diagnosis} and \texttt{medication} have the same cardinality $n$. The number of operations needed to evaluate the query is $\mathcal{O}(n^2)$ 
%(due to the oblivious $\theta$-join) 
whereas the number of communication rounds is $\mathcal{O}(\log^2 n)$.
% (due to oblivious sorting). 
%The space requirements are again bounded by the size of the two input relations, i.e. $\mathcal{O}(n)$. 
In contrast, an end-to-end oblivious implementation of the plan in \cite{Bater2017SMCQL} requires 
%$\mathcal{O}(n^2)$ space (to materialize the join output), 
$\mathcal{O}(n^2\log^2 n)$ operations and $4\times$ more rounds, since it applies distinct to the materialized join output.

%Synthetic data (?)


%\stitle{Query 1 (Comorbidity).} In the first step, we evaluate the \texttt{IN} operator to identify rows whose \texttt{pid} appears in \texttt{cohort}. This step appends a new column of single-bit shares to \texttt{diagnosis}, as described in Section~\ref{sec:secure_operators}. In the second step, we apply the \texttt{GROUP-BY} operator, which updates \texttt{diagnosis} in-place by sorting it on the attribute \texttt{diag} and counting the number of rows in each group. To do so, the \texttt{GROUP-BY} operator takes into account the bit shares generated by the selection of the previous step, as described in Section~\ref{sec:constructing_plans}. \john{FUSION} 
%The third phase of \texttt{GROUP-BY} (shuffling) is omitted in this query since \texttt{diagnosis} is sorted again in the next step (on the resulting \texttt{cnt} values) to apply the final \texttt{ORDER-BY}. When done with this last step, each computing party simply opens the first ten rows of \texttt{diagnosis}. 
%
%\vasia{Figure~}\ref{fig:opt-plans}.
%
%\emph{To summarize, the number of operations needed to evaluate \texttt{Q1} is $\mathcal{O}(n\log^2 n)$ -- due to oblivious sorting -- whereas the number of communication rounds is $\mathcal{O}(n)$ -- due to oblivious grouping. %,  where $n$ is the cardinality of \texttt{diagnosis}. 
%The space requirements are bounded by the size of \texttt{diagnosis}, i.e., $\mathcal{O}(n)$.}
%
%\mv{An alternative plan to calculate the count of the GROUP-BY with $O(log n)$ communication rounds, although with high computational cost. Start with the same first step as needed to compute the DISTINCT operator: obliviously create a vector $\vec{v}$ where each value $v_i$ indicates whether relation $i$ is different than the relation before it (the equality check is a $O(log n)$ operation, and all of them can be done in parallel). Next create the vector $\vec{w}$ of prefix sums of $\vec{v}$, i.e., $w_i = \sum_{j=1}^{i}{v_j}$. This vector has the form $\langle 1, 1, \ldots, 1, 2, \ldots, 2, 3, \ldots \rangle$, and it indicates that position $i$ contains the $w_i^{\text{th}}$ distinct value. In parallel, compute whether each $w_i$ value is equal to $1, 2, \ldots, n$ and sum up these numbers to determine the counts of the 1st, 2nd, $\ldots$, nth distinct elements.}
%
%\stitle{Query 2 (Recurrent C. Diff.).} This query is a bit more complex than \texttt{Q1} and requires careful evaluation. \texttt{Q2} includes a nested query (that generates a relation \texttt{rcd}), followed by a self-join of \texttt{rcd} and a \texttt{DISTINCT} operator on the output of the join. A baseline evaluation would apply \texttt{DISTINCT} on the self-join output, which in turn requires materializing and sorting the cartesian product $\texttt{rcd}\times\texttt{rcd}$. Our evaluation plan avoids this expensive operation as follows. 
%
%In the first step, we evaluate the selection predicate \texttt{diag~=~cdiff} to identify patients diagnosed with \texttt{C. Diff}. This step appends one column of single-bit shares to \texttt{diagnosis}. Let $s_i$ be the share of the selection result (0/1) for the $i$-th row. In the second step, we order \texttt{diagnosis} first on \texttt{pid} and then on (ascending) \texttt{time}. Intuitively, this operation `clusters' each patient's records in consecutive rows ordered by \texttt{time}.
%Next, we scan \texttt{diagnosis} and apply the \texttt{DISTINCT} predicate on-the-fly along with the two inequality predicates (\texttt{r2.time - r1.time $\geq$ 15 DAYS} and \texttt{r2.time - r1.time $\leq$ 56 DAYS}) on each pair of adjacent rows. This step checks $n-1$ pairs in total, where $n$ is the cardinality of \texttt{diagnosis}; however, it can be done in constant number of rounds since each check is independent of the others. 
%A single application of the two inequality predicates includes two boolean additions followed by two inequality checks. 
%Let $d_i$ be the bit share generated by \texttt{DISTINCT}, and $g_i$, $g'_i$ be the result share for the respective inequality check. For each row $i$, we evaluate the logical formula  $d_i~\texttt{AND}~g_i~\texttt{AND}~g'_i~\texttt{AND}~s_i$ and write back the result to $s_i$. Then, we sort \texttt{diagnosis} first on $s_i$ and then on \texttt{pid}. In the final step, we scan \texttt{diagnosis} and evaluate the logical expression $s_i~\texttt{AND}~s_{i+1}$ on each pair of adjacent rows, storing the result back in $s_i$. Note that, in this final step, we compare adjacent rows so there is no need to evaluate the predicate \texttt{r2.row\_no = r1.row\_no + 1} under MPC, which is simply omitted. In the end, each computing party opens all rows in \texttt{diagnosis}.  
%
%\emph{To summarize, the number of operations needed to evaluate \texttt{Q2} is $\mathcal{O}(n\log^2 n)$ whereas the number of communication rounds is $\mathcal{O}(\log^2 n)$, both due to oblivious sorting. The space requirements are again bounded by the size of \texttt{diagnosis}, i.e. $\mathcal{O}(n)$. In contrast, the baseline plan would have $\mathcal{O}(n^2)$ space requirements and would need $\mathcal{O}(n^4\log^2 n)$ operations and $\mathcal{O}(\log^2 n)$ rounds. This is because partitioning is not possible under MPC without revealing the group sizes.}
%
%\stitle{Query 3 (Aspirin Count).}
%\texttt{Q3} includes a $\theta$-join between two relations \texttt{diagnosis} and \texttt{medication} and a \texttt{COUNT(DISTINCT)} aggregation on the join output. In this case, our evaluation plan pushes the (blocking) \texttt{DISTINCT} operator before the join to avoid materializing and sorting the join output. The evaluation works as follows. 
%
%First, we apply the selection predicates \texttt{d.diag~=~hd} and \texttt{m.med = aspirin} on \texttt{diagnosis} and \texttt{medication} respectively. Each of these selections appends a new column of single-bit shares to the corresponding relation. Let $s_i$ be the share of the selection result (0/1) for the $i$-th row of each relation. 
%In the second step, we sort each relation first on $s_i$, then on \texttt{pid}, and then on \texttt{time} (ascending for  \texttt{diagnosis} and descending for \texttt{medication}). These two oblivious sortings can be done in parallel as they do not depend on each other. Then, we scan each relation and apply the \texttt{DISTINCT} operator, which generates one single-bit share for each row. Let $d_i$ be the \texttt{DISTINCT} bit for row $i$. In the final step, we perform a nested-loop join between the two relations and, for each pair ($i, j$), we evaluate the formula $s_i~\texttt{AND}~d_i~\texttt{AND}~s_j~\texttt{AND}~d_j~\texttt{AND}~\texttt{d.time}~\leq~\texttt{m.time}$ on-the-fly, and open the corresponding pair. 
%
%\emph{To summarize, the number of operations needed to evaluate \texttt{Q2} is $\mathcal{O}(n^2)$ -- due to the oblivious join -- whereas the number of communication rounds is $\mathcal{O}(\log^2 n)$ -- due to oblivious sorting. The space requirements are again bounded by the size of the input, i.e. $\mathcal{O}(n)$, since the join can be done in a pipelined fashion. In contrast, the baseline plan would have $\mathcal{O}(n^2)$ space requirements (to materialize the join output) and would need $\mathcal{O}(n^2\log^2 n)$ operations and $\mathcal{O}(\log^2 n)$ rounds.}


